Knowing The What But Not The Where in Bayesian Optimization

Bayesian optimization has demonstrated impressive success in finding the optimum input x* and output f* = f(x*) = max f(x) of a black-box function f. In some applications, however, the optimum output f* is known in advance and the goal is to find the corresponding optimum input x*. In this paper, we consider a new setting in BO in which the knowledge of the optimum output f* is available. Our goal is to exploit the knowledge about f* to search for the input x* efficiently. To achieve this goal, we first transform the Gaussian process surrogate using the information about the optimum output. Then, we propose two acquisition functions, called confidence bound minimization and expected regret minimization. We show that our approaches work intuitively and give quantitatively better performance against standard BO methods. We demonstrate real applications in tuning a deep reinforcement learning algorithm on the CartPole problem and XGBoost on Skin Segmentation dataset in which the optimum values are publicly available.

==> Acquisition_Derivation.tex <==
Let $\mathcal{D}_{t}=\left\{ x_{i}\in\mathcal{R}^{d},y_{i}\in\mathcal{R}\right\} _{i=1}^{t}$
be the observation set including a feature $x_{i}$ and an outcome
$y_{i}$. We define the regret function $r\left(x\right)=f^{*}-f(x)$
where $f^{*}$ is the known global optimum value. The likelihood of
improvement $r\left(x\right)$ (for brevity, we write $r$) on a normal
posterior distribution is as follows
\begin{align}
p\left(r\right)= & \frac{1}{\sqrt{2\pi}\sigma\left(x\right)}\exp\left(-\frac{1}{2}\frac{\left[\mu\left(x\right)-f^{*}+r\right]^{2}}{\sigma^{2}\left(x\right)}\right).\label{eq:ELI_llk_improvement}
\end{align}
Our acquisition function (to be minimized) is then defined as $\alpha\left(x\right)=\mathbb{E}\left[G\left(x\right)\right]$.
Using the likelihood function in Eq. (\ref{eq:ELI_llk_improvement}),
we obtain 
\begin{align*}
\alpha\left(x\right) & =\int_{0}^{\infty}\frac{r}{\sqrt{2\pi}\sigma\left(x\right)}\exp\left(-\frac{1}{2}\frac{\left[\mu\left(x\right)-f^{*}+r\right]^{2}}{\sigma^{2}\left(x\right)}\right)dr.
\end{align*}
Let $t=\frac{\mu\left(x\right)-f^{*}+r}{\sigma\left(x\right)}$, then
$r=t\times\sigma\left(x\right)-\mu(x)+f^{*}$ and $dt=\frac{dG}{\sigma\left(x\right)}$.
We write $\alpha\left(x\right)$ as
\begin{align}
\alpha\left(x\right) & =\int_{t=\frac{\mu\left(x\right)-f^{*}}{\sigma\left(x\right)}}^{\infty}\frac{\left(t\times\sigma\left(x\right)+f^{*}-\mu\left(x\right)\right)}{\sqrt{2\pi}\sigma\left(x\right)}\exp(-\frac{1}{2}t^{2})\times\sigma\left(x\right)dt\nonumber \\
 & =\sigma\left(x\right)\int_{t=\frac{\mu\left(x\right)-f^{*}}{\sigma\left(x\right)}}^{\infty}\frac{t}{\sqrt{2\pi}}\exp(-\frac{1}{2}t^{2})dt+\left[f^{*}-\mu\left(x\right)\right]\int_{t=\frac{\mu\left(x\right)-f^{*}}{\sigma\left(x\right)}}^{\infty}\frac{1}{\sqrt{2\pi}}\exp(-\frac{1}{2}t^{2})dt.\label{eq:alpha_EI_derivation}
\end{align}
We compute the first term in Eq. (\ref{eq:alpha_EI_derivation}) as
follows
\begin{align*}
\sigma\left(x\right)\int_{t=\frac{\mu\left(x\right)-f^{*}}{\sigma\left(x\right)}}^{\infty}\frac{t}{\sqrt{2\pi}}\exp(-\frac{1}{2}t^{2})dt & =\frac{\sigma\left(x\right)}{\sqrt{2\pi}}\left[-\exp\left(-\frac{1}{2}\left[\frac{\mu\left(x\right)-f^{*}+r}{\sigma\left(x\right)}\right]^{2}\right)\right]_{r=0}^{r=\infty}\\
 & =\sigma(x)\mathcal{N}\left(\frac{\mu\left(x\right)-f^{*}}{\sigma\left(x\right)}\mid0,1\right).
\end{align*}
We compute the second term in Eq. (\ref{eq:alpha_EI_derivation})
as 
\begin{align*}
\left[f^{*}-\mu\left(x\right)\right]\int_{t=\frac{\mu\left(x\right)-f^{*}}{\sigma\left(x\right)}}^{\infty}\frac{1}{\sqrt{2\pi}}\exp(-\frac{1}{2}t^{2})dt & =\left[f^{*}-\mu\left(x\right)\right]\left\{ \int_{-\infty}^{\infty}\mathcal{N}\left(t\mid0,1\right)dt-\int_{-\infty}^{\frac{\mu\left(x\right)-f^{*}}{\sigma\left(x\right)}}\mathcal{N}\left(t\mid0,1\right)dt\right\} \\
 & =\left[f^{*}-\mu\left(x\right)\right]\left[1-\Phi\left(\frac{\mu\left(x\right)-f^{*}}{\sigma\left(x\right)}\right)\right].
\end{align*}
Explicitly, denoting $z=\frac{\mu\left(x\right)-f^{*}}{\sigma\left(x\right)}$,
we obtain the acquisition function as follows
\begin{align}
\alpha\left(x\right) & =\sigma\left(x\right)\phi\left(z\right)+\left(f^{*}-\mu\left(x\right)\right)\left(1-\Phi\left(z\right)\right)\label{eq:AcqFunc_ELI}
\end{align}
where $\phi\left(z\right)=\mathcal{N}\left(z\mid0,1\right)$ is the
standard normal pdf and $\Phi\left(z\right)$ is the cdf.

To select the next point, we minimize this acquisition function
\begin{align*}
x_{t+1} & =\arg\min_{x\in\mathcal{X}}\alpha(x)
\end{align*}

We can see that this acquisition function is minimized $\alpha(x)=0$
when $f^{*}-\mu(x)=0$ and $\sigma(x)=0$.

We consider the special case when $\sigma(x)=0$:

Since the case of $\mu(x)>f^{*}$ and $\sigma(x)=0$ will not happen
because $f^{*}\ge f(x),\forall x\in\mathcal{X}$, we consider the
second case as $\mu(x)\le f^{*}$, then $z=-\infty$, $\Phi\left(z\right)=0$,
$\phi(z)=0$, $\alpha(x)\sim f^{*}-\mu(x)$.




==> Introduction.tex <==
The optimization of an unknown function based on noisy observations
is a fundamental problem in various real world domains, e.g., engineering
design {[}34{]}, finance {[}37{]} and hyper-parameter optimization
{[}30{]}. In recent years, an increasingly popular direction has been
to model smoothness assumptions about the function via a Gaussian
Process (GP), which provides an easy way to compute the posterior
distribution of the unknown function, and thereby uncertainty estimates
that help to decide where to evaluate the function next, in search
of an optima. This Bayesian optimization (BO) framework has received
considerable attention in tuning of hyper-parameters for complex models
and algorithms in Machine Learning, Robotics and Computer Vision {[}16,
32, 30, 12{]}.

While the goal of Bayesian optimization is to keep the number of evaluations
of f as low as possible, in highdimensional and or otherwise complex
problems, the number of required evaluations can still be considerable.
Parallel approaches arise as the natural solution to circumvent the
computational bottleneck around these evaluations of f. While in practice,
we can often evaluate several different choices in parallel, such
as multiple machines can simultaneously train the machine learning
algorithm with different sets of hyperparameters. Such scenarios appear,
for instance, in the optimization of computer models where several
cores are available to run in parallel, or in wet-lab experiments
when the cost of testing one experimental design is the same as testing
a batch of them.

\subsection*{Related work}

\input{RelatedWork.tex}

\subsection*{Contribution}

Motivated by this line of work in batch BO, we propose in this paper
a new approach which utilizes the geometric distance of the observations
for exploration.


==> Introduction_1.tex <==
Bayesian Optimization (BO) is an efficient method for global optimization
of a black-box function using noisy point-wise observations. BO has
been employed in selection of chemical compounds \cite{Hernandez_2017Parallel},
online marketing {[}43{]}, reinforcement learning problems {[}15,
29{]}, and in search for hyperparameters of machine learning algorithms
\cite{klein2017fast}. 

Bayesian optimization incorporates prior belief about f and updates
the prior with samples drawn from f to get a posterior that better
approximates f. The model used for approximating the objective function
is called surrogate model. A popular choice for a surrogate model
is a Gaussian process (GP), a generalization of Gaussian random vector
to the space of functions.

BO requires a probabilistic model that reliably models the uncertainty
in the unexplored part of the domain of the black-box function. This
model is used to define an acquisiton function whose maximum determines
the next sequential query of black-box function. Bayesian optimization
also uses an acquisition function that directs sampling to areas where
an improvement over the current best observation is likely.

{[}BO{]} Bayesian optimization (BO) has received considerable attention
in tuning hyper-parameters for complex models and algorithms \cite{Brochu_2010Tutorial,Hennig_2012Entropy,Snoek_2012Practical,Shahriari_2016Taking}.
In a standard setting, BO suggests one evaluation at a time, whereas
batch BO can recommend multiple evaluations where parallel facilities
are available. The batch setting is essential to speed up the optimization
process. Such scenarios appear, for instance, in optimizing computer
models where several cores are available for parallel runs. Another
example is in wet-lab experiments, wherein the need for batch experiments
is significant as the cost of testing one experiment is the same as
testing a batch.

Global optimization of such functions is close to impossible without
any further assumption on $f$. A common assumption is a Gaussian
Process (GP) prior on the function $f$, which ensures a degree of
smoothness of $f$. Although this is an old idea dating back to ,
there has been considerable attention in the recent past .

Thompson sampling is a useful tool for exploration. Drawing a Gaussian
process instance given the existing observations. Ideally, if we can
estimate the true hyper-parameter of a GP kernel, we can simply selecting
the location which maximizes the GP mean function. Unfortunately,
estimating the hyperparameters of GP kernels with very few function
evaluations is a challenging task, often with disastrous consequences
as illustrated by a simple example in \cite{benassi2011robust}. The
typical estimation of the hyperparameters by maximizing the marginal
likelihood \cite{Jones_1998Efficient,Rasmussen_2006gaussian}, can
easily fall into traps, as shown in \cite{Bull_2011Convergence}.
Several authors have proposed to integrate out the hyperparameters
using quadrature or MC methods \cite{Brochu_2010Tutorial,Snoek_2012Practical}.
These more advanced techniques can still fall in traps as illustrated
with a simple simulation example in \cite{Wang_2014Theoretical},
where theoretical bounds are used to ensure that Bayesian optimization
is robust with respect to the choice of hyperparameters.

In this paper, we consider batch Bayesian optimization problem for
situations where the black-box function evaluation is less expensive.
To make batch BO efficient, we propose a new exploration strategy,
called \emph{distance exploration,} which utilizes the geometric distance
of the observations for exploration rather than the Gaussian process
(GP) predictive variance. Our intuition for distance exploration is
based on the fact that the best location for exploration should not
be close to the existing observations. 

Based on the proposed \emph{distance exploration}, we present a simple,
but effective approach for batch Bayesian optimization. In our algorithm,
we follow a common setting \cite{Desautels_2014Parallelizing,Contal_2013Parallel,Gonzalez_2015Batch,Kathuria_NIPS2016Batched}
to select the first item in a batch following the standard BO. The
remaining elements are selected by the proposed \emph{distance exploration.}
 We show that our distance exploration is a special case of using
the GP predictive variance. We derive the sublinear convergence analysis
for the proposed approach. We validate our model using an extensive
set of benchmark functions and selected real-world applications which
are less expensive. These experiments demonstrate that our distance
exploration (DE) approach outperforms all the baselines in terms of
computation while being competitive in finding the optimal value against
the baselines. 

Our main contributions are
\begin{itemize}
\item A first study of Bayesian optimization to incorporate known optimum
value.
\item We propose Thompson sampling approaches for sequential and batch BO
given known optimum value.
\item We evaluate the performance of our approaches in several benchmark
functions and real-world experiments. 
\end{itemize}


